Don't Judge Before You CLIP: A Unified Approach for Perceptual Tasks

Visual perceptual tasks aim to predict human judgment of images (e.g., emotions invoked by images, image quality assessment). Unlike objective tasks such as object/scene recognition, perceptual tasks rely on subjective human assessments, making its data-labeling difficult. The scarcity of such human-annotated data results in small datasets leading to poor generalization. Typically, specialized models were designed for each perceptual task, tailored to its unique characteristics and its own training dataset. We propose a unified architectural framework for solving multiple different perceptual tasks leveraging CLIP as a prior. Our approach is based on recent cognitive findings which indicate that CLIP correlates well with human judgment. While CLIP was explicitly trained to align images and text, it implicitly also learned human inclinations. We attribute this to the inclusion of human-written image captions in CLIP's training data, which contain not only factual image descriptions, but inevitably also human sentiments and emotions. This makes CLIP a particularly strong prior for perceptual tasks. Accordingly, we suggest that minimal adaptation of CLIP suffices for solving a variety of perceptual tasks. Our simple unified framework employs a lightweight adaptation to fine-tune CLIP to each task, without requiring any task-specific architectural changes. We evaluate our approach on three tasks: (i) Image Memorability Prediction, (ii) No-reference Image Quality Assessment, and (iii) Visual Emotion Analysis. Our model achieves state-of-the-art results on all three tasks, while demonstrating improved generalization across different datasets.

==> tables/EMO_single.tex <==
\begin{table}[!h]
\centering
\resizebox{0.43\textwidth}{!}{%
\begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} 
    & \multicolumn{2}{c}{\textbf{EmoSet}} 
    & \multicolumn{2}{c}{\textbf{EmotionROI}} \\ 
    \cmidrule(r){2-3} 
    \cmidrule(r){4-5}  
    & \textbf{8} & \textbf{2} 
    & \textbf{6} & \textbf{2}  \\ 
    \midrule
    MRCNN  
    & 0.7539 & 0.9228  
    & - & -  \\ 
    MDAN  
    & 0.7575 & 0.9371  
    & 0.6166 & -  \\ 
    StimuliVEA  
    & 0.7840 & 0.9458  
    & 0.6162 & -  \\ 
    PT-DPC  
    & 0.7713 & 0.9246  
    & 0.6970 & 0.8855  \\ 
    SimEmotion  
    & 0.7906 & 0.9428  
    & 0.7054 & 0.9040  \\ 
    MVP
    & 0.8192 & 0.9644  
    & 0.7189 & 0.9255  \\ 
    \midrule
    \textbf{PerceptCLIP (Ours)}  
    & \textbf{0.8528} & \textbf{0.9780}  
    & \textbf{0.7485} & \textbf{0.9288}  \\ 
    \bottomrule
\end{tabular}
}
\parbox{0.43\textwidth}{\caption{\textbf{Model Performance on Emotion Classification.} Accuracy results for binary and multi-class emotion classification on the EmotionROI (mean over five splits) and EmoSet datasets. 
Our model achieves state-of-the-art performance for both datasets.
} 
\label{tab:EMO_single}}
\end{table}

==> tables/MEM_single.tex <==
\begin{table}[th!]
\centering
\resizebox{0.36\textwidth}{!}{%
\begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} 
    & \multicolumn{2}{c}{\textbf{LaMem}} \\
    \cmidrule(r){2-3} 
    & {SRCC$\uparrow$} & {MSE$\downarrow$} \\
    \midrule
    MemNet  
    & 0.640 & Unknown \\
    AMNet  
    & 0.677 & 0.0082  \\
    Leonardi et al  
    & 0.687 & 0.0079  
     \\ 
    ViTMem  
    & 0.711 & 0.0076  
      \\ 
    Squalli-Houssaini et al
    & 0.720 & 0.0092  
    \\ 
    \midrule
    \textbf{PerceptCLIP (Ours)}  
    & \textbf{0.741} & \textbf{0.0069} \\ 
    \bottomrule
\end{tabular}
}
\parbox{0.36\textwidth}{\caption{\textbf{Model Performance on Image Memorability.} Average SRCC and MSE across 5 splits of the LAMEM dataset are reported, 
showing that our model, PerceptCLIP, surpasses all previous methods.}
\label{tab:MEM_single}}
\end{table}

==> tables/abl_clip_sizes_and_bacbones.tex <==
\begin{table*}[h!]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccccc}
            \toprule
            \multirow{3}{*}{\textbf{Backbone}} 
            & \multicolumn{2}{c}{\textbf{IQA}}  
            & \textbf{VEA} 
            & \multicolumn{2}{c}{\textbf{Memorability}} \\
            & \multicolumn{2}{c}{KonIQ-10k}  
            & EmoSet-8 
            & \multicolumn{2}{c}{LaMem} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6} 
            & {SRCC$\uparrow$} & {PLCC$\uparrow$} 
            & {ACC$\uparrow$} 
            & {SRCC$\uparrow$} & {MSE$\downarrow$} \\
            \midrule
                \textbf{MAE} 
            & {0.924} & {0.935} 
            & {0.7681} 
            & {0.699} & {0.0078} \\
            \textbf{DinoV2} 
            & {0.937} & {0.950} 
            & {0.8252} 
            & {0.729} & {0.0071} \\
                \textbf{CLIP} 
            & \textbf{0.945} & \textbf{0.954} 
            & \textbf{0.8528} 
            & \textbf{0.741} & \textbf{0.0069} \\
        
            \bottomrule
        \end{tabular}%
        }
        \caption{\textbf{Effect of Vision Backbones on Performance:} We trained our model with different backbones, applying LoRA to the q, k, and v layers. CLIP outperforms MAE and DINOv2 across all tasks, demonstrating its stronger perceptual prior.}
        \label{tab:backbone}
    \end{minipage}
    \hfill
    \begin{minipage}{0.48\textwidth}
        \centering
        \resizebox{\textwidth}{!}{%
        \begin{tabular}{lcccccc}
            \toprule
            \multirow{2}{*}{\textbf{Method}} 
            & \multicolumn{2}{c}{\textbf{IQA}}  
            & \textbf{VEA} 
            & \multicolumn{2}{c}{\textbf{Memorability}} \\
            & \multicolumn{2}{c}{KonIQ-10k}  
            & EmoSet-8 
            & \multicolumn{2}{c}{LaMem} \\
            \cmidrule(lr){2-3} \cmidrule(lr){4-4} \cmidrule(lr){5-6} 
            & {SRCC$\uparrow$} & {PLCC$\uparrow$} 
            & {ACC$\uparrow$} 
            & {SRCC$\uparrow$} & {MSE$\downarrow$} \\
            \midrule
            \textbf{ViT-B/32} 
            & 0.932 & 0.944 
            & 0.8303 
            & 0.724 & 0.0073 \\
            \textbf{ViT-B/16} 
            & {0.938} & {0.949} 
            & {0.8422} 
            & 0.731 & 0.0071 \\
            \textbf{ViT-L/14} 
            & \textbf{0.945} & \textbf{0.954} 
            & \textbf{0.8528} 
            & \textbf{0.741} & \textbf{0.0069} \\
            \bottomrule
        \end{tabular}%
        }
        \caption{\textbf{Performance of Different CLIP Variants:} We trained our model using different sizes of ViT as the CLIP vision encoder. The results show that ViT-B/16 outperforms ViT-B/32, suggesting that a finer patch resolution improves perceptual understanding. ViT-L/14 achieves the best overall performance, reinforcing its use as our backbone model.}
        \label{tab:clip_sizes}
    \end{minipage}
\end{table*}


==> tables/abl_lora_config.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lccc}
    \toprule
    \diagbox{{r}}{\textbf{$\alpha$}} 
    & \textbf{4} & \textbf{8} & \textbf{16} \\
    \midrule
    \textbf{8}  & 0.945 & 0.944 & 0.944 \\
    \textbf{16} & 0.944 & 0.945 & 0.945 \\
    \textbf{32} & 0.945 & 0.944 & 0.944 \\
    \bottomrule
\end{tabular}%
\caption{\textbf{SRCC Performance Across LoRA Configurations:} Spearman Rank Correlation Coefficient (SRCC) values for different combinations of LoRA rank ($r$) and scaling factor ($\alpha$) on the \textbf{kon10k dataset} within the IQA task.}
\label{tab:lora_srcc}
\end{table}

\begin{table}[h!]
\centering
\begin{tabular}{lccc}
    \toprule
    \diagbox{{r}}{\textbf{$\alpha$}} 
    & \textbf{4} & \textbf{8} & \textbf{16} \\
    \midrule
    \textbf{8}  & 0.954 & 0.954 & 0.954 \\
    \textbf{16} & 0.954 & 0.954 & 0.954 \\
    \textbf{32} & 0.954 & 0.953 & 0.953 \\
    \bottomrule
\end{tabular}%
\caption{\textbf{PLCC Performance Across LoRA Configurations:} Pearson Linear Correlation Coefficient (PLCC) values for different combinations of LoRA rank ($r$) and scaling factor ($\alpha$) on the \textbf{kon10k dataset} within the IQA task.}
\label{tab:lora_plcc}
\end{table}


==> tables/all_results.tex <==
\begin{table}[b!]
\centering 
\resizebox{0.48\textwidth}{!}{%

\begin{tabular}{cc|cc|cc}
    \toprule
    \multicolumn{2}{c|}{\textbf{IQA (LIVEC)}} 
    & \multicolumn{2}{c|}{\textbf{VEA (EmoROI-6)}} 
    & \multicolumn{2}{c}{\textbf{Memorability (LaMem)}} \\
    \cmidrule(r){1-2} \cmidrule(r){3-4} \cmidrule(r){5-6}
    \textbf{Method} & \textbf{PLCC} 
    & \textbf{Method} & \textbf{ACC} 
    & \textbf{Method} & \textbf{SRCC} \\ 
    \midrule
    LoDA & {0.899} 
        & PT-DPC & {0.697} 

    & Leonardi et al& 0.687 \\
    LIQE & 0.910 
    & SimEmotion & 0.705 
    & ViTMem & 0.711 \\
    QPT-ResNet50 & {0.914} 

    & MVP & {0.719} 

    & Squalli-Houssaini et al& {0.720} \\
    \midrule
    \textbf{Ours} & \textbf{0.923} 
    & \textbf{Ours} & \textbf{0.749} 
    & \textbf{Ours} & \textbf{0.741} \\
    \textbf{Ours Multi} & \textbf{0.933} 
    & \textbf{Ours Multi} & \textbf{0.759} 
    & \textbf{Ours Multi} & \textbf{0.740} \\
    \bottomrule
\end{tabular}}
\caption{}
\label{tab:all_results}
\end{table}

==> tables/multi_EMO.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcc}
    \toprule
    {\textbf{Method}} 
    & {\textbf{EmoSet-8}} 
    & {\textbf{EmotionROI-6}} \\   
    \midrule
    \textbf{Ours}  
    & \textbf{0.8528} 
    & {0.7485}  \\ 
    \textbf{Ours Multi}  
    & {0.8511}  
    & \textbf{0.7591}   \\ 
    \bottomrule
\end{tabular}
\caption{\textbf{Multi-Dataset vs. Single-Dataset Training for Emotion Recognition:} Training EmotionROI-6 togther with EmoSet-8 improves performance on EmotionROI-6 while maintaining comparable results to single-dataset training on EmoSet-8.}
\label{tab:Multi_EMO}
\end{table}

==> tables/multi_MEM.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lcccc}
    \toprule
    \multirow{2}{*}{\textbf{Method}} 
    & \multicolumn{2}{c}{\textbf{LaMem}} 
    & \multicolumn{2}{c}{\textbf{THINGS}} \\ 
    \cmidrule(r){2-3} 
    \cmidrule(r){4-5}  
    & {SRCC} & {MSE} 
    & {SRCC} & {MSE}  \\ 
    \midrule
    \textbf{Ours}  
    & \textbf{0.741} & \textbf{0.0069}  
    & {0.452} & {0.0058}  \\
        \textbf{Ours Multi}  
    & {0.740} & \textbf{0.0069}  
    & \textbf{0.454} & \textbf{0.0054}  \\
    \bottomrule
\end{tabular}
\caption{\textbf{Multi-Dataset vs. Single-Dataset Training for Memorability Prediction:} The multi-dataset approach improves performance on THINGS while maintaining comparable results on LaMem.}
\label{tab:Multi_MEM}
\end{table}
